An Investigation of Warning Erroneous Chat Translations in Cross-lingual Communication

Machine translation models are still inappropriate for translating chats, despite the popularity of translation software and plug-in applications. The complexity of dialogues poses significant challenges and can hinder crosslingual communication. Instead of pursuing a flawless translation system, a more practical approach would be to issue warning messages about potential mistranslations to reduce confusion. However, it is still unclear how individuals perceive these warning messages and whether they benefit the crowd. This paper tackles to investigate this question and demonstrates the warning messages' contribution to making chat translation systems effective.

==> figures/q1_summary.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/q1_summary.png}
\caption{The results of the feedback question about whether participants think there were erroneous translations in the chat without hints.}
\label{fig:q1}
\end{figure}
